On the Uncertain Single-View Depths in Colonoscopies

Estimating depth information from endoscopic images is a prerequisite for a wide set of AI-assisted technologies, such as accurate localization and measurement of tumors, or identification of non-inspected areas. As the domain specificity of colonoscopies -- deformable low-texture environments with fluids, poor lighting conditions and abrupt sensor motions -- pose challenges to multi-view 3D reconstructions, single-view depth learning stands out as a promising line of research. Depth learning can be extended in a Bayesian setting, which enables continual learning, improves decision making and can be used to compute confidence intervals or quantify uncertainty for in-body measurements. In this paper, we explore for the first time Bayesian deep networks for single-view depth estimation in colonoscopies. Our specific contribution is two-fold: 1) an exhaustive analysis of scalable Bayesian networks for depth learning in different datasets, highlighting challenges and conclusions regarding synthetic-to-real domain changes and supervised vs. self-supervised methods; and 2) a novel teacher-student approach to deep depth learning that takes into account the teacher uncertainty.

==> Sections/suplementary.tex <==
\section*{On the Uncertain Single-View Depths in Colonoscopies -Supplementary Material-}
\pagenumbering{gobble} 
\setcounter{page}{1}
\setcounter{figure}{0}
\begin{figure}%{\textwidth}
  \includegraphics[width=\columnwidth]{img/Train-SL.pdf}
  \centering
  \caption{Supervised training of a single ensemble \textit{m}. Depth $\widehat{d}_m$ and aleatoric uncertainty $\sigma_{a,m},$ estimation for a target image $\mathcal{I}$. We define graphically the loss for a single ensemble. $\widehat{d}_m$ depth prediction, $d$ depth target  and $\sigma_{a,m}$ the aleatoric uncertainty of the ensemble. }
\label{fig:trainsup}
\end{figure}

\begin{figure}
    \centerline{\includegraphics[width=\columnwidth]{img/Train-SSL.pdf}}
    \caption{Self-supervised training of deep ensembles. Each network $m$ in the ensemble learns to predict disparity $\widehat{\underline{d}}$ and observation noise $\widehat{u}_m$, referred to photometric residual, for a target image $\mathcal{I}_i$. A secondary network predicts the relative rotation $\boldsymbol{R}$ and translation $\boldsymbol{t}$ between the target view and several source ones $\mathcal{I}_{i^\prime}$. The predicted depths and camera motion allows to warp the target image to the image plane of the source images $\mathcal{I}_{i^\prime\rightarrow i}$. The loss $\mathcal{L}_m$ depends on a function of the three color images.}
    \label{fig:Approach_Self-Supervised}
\end{figure}
\begin{figure}
    \centerline{\includegraphics[width=\columnwidth]{img/Train_self-teaching_learning.pdf}}
    
 \caption{Self-supervised training by a teacher-student approach. An ensemble of $M$ deep networks (teacher) supervises the training of a single encoder-decoder (student).
     Our contribution to improve the the state of the art is summing up the teacher's total uncertainty $\widehat{\sigma}_{t,T}$ to the aleatoric uncertainty issued by the student network $\widehat{\sigma}_{a}$ to obtain the depth error variance $\widehat{\sigma}_{S}$ that is included in the loss.
     }
    \label{fig:Approach_Teacher}
\end{figure}

\begin{figure}{\columnwidth}
  \centering
  \includegraphics[width=0.7\columnwidth]{img/colmap-real.png}
  \caption{Multi-view reconstruction from the real colonoscopy images of the EndoMapper project using COLMAP.}
\end{figure}
\begin{figure}{\columnwidth}
  \centering
  \includegraphics[width=0.45\columnwidth,angle=90]{img/Selection_111.png}
  \caption{ Multi-view reconstruction from the colonoscopy synthetic images using COLMAP.
  }
    \label{fig:colmap-synth}
\end{figure}
